Ice-Breakers, Turn-Takers and Fun-Makers: Exploring Robots for Groups with Teenagers

Successful, enjoyable group interactions are important in public and personal contexts, especially for teenagers whose peer groups are important for self-identity and self-esteem. Social robots seemingly have the potential to positively shape group interactions, but it seems difficult to effect such impact by designing robot behaviors solely based on related (human interaction) literature. In this article, we take a user-centered approach to explore how teenagers envisage a social robot "group assistant". We engaged 16 teenagers in focus groups, interviews, and robot testing to capture their views and reflections about robots for groups. Over the course of a two-week summer school, participants co-designed the action space for such a robot and experienced working with/wizarding it for 10+ hours. This experience further altered and deepened their insights into using robots as group assistants. We report results regarding teenagers' views on the applicability and use of a robot group assistant, how these expectations evolved throughout the study, and their repeat interactions with the robot. Our results indicate that each group moves on a spectrum of need for the robot, reflected in use of the robot more (or less) for ice-breaking, turn-taking, and fun-making as the situation demanded.

==> sections/05_codesign.tex <==
% done grammarly
\section{Co-design and articulation of social robot behaviors}
A core element of our efforts to include teenagers in the design and discussion of social robot behaviours was to co-design the robot's non-verbal and verbal communication abilities. As we embedded the study in a two-week summerschool, we decided to constrain the design of the behaviour to discrete actions, i.e. 'Say hello' or 'Nod'. Further, we limited the design of behaviours to the NAO robot, a robot commonly used in child-robot educational contexts (e.g. ~\cite{senft2019teaching,kennedySocialRobotTutoring2016,lemaignanLearningTeachingRobot2016,alves-oliveiraEmpathicRobotGroup2019}). %While we exposed participants to different social robots during the initial co-design sessions, 
We chose to constrain the designed actions and the robot to implement the designed actions on the robot rapidly. This way we could ensure that teenagers could fully experience the robot's behaviours they designed and reflect upon them.


\subsection{Methodology}\label{sec:comethodlogy}
\subsubsection{Group Communication and `Robot' Assistant Activities and Games}
Ahead of starting detailed action space co-design, we undertook a number of reflective activitiesfirst to get participants thinking about multimodal communication in groups; specifically how one member's behaviours can influence the group experience and how robots might need to be explicitly programmed to do, e.g. nonverbal behaviours we often take for granted. %In order to prompt the students to think (specifically multimodal) behaviour in groups, we undertook a number of group, game-like activities whereby they had to reflect on their own and/or the group's behaviour. 
These included:
\begin{itemize}
    \item an adapted version of the `telephone game'~\footnote{\url{https://en.wikipedia.org/wiki/Chinese_whispers}} where participants had to pass a message between themselves each person using a different modality (movement, facial expression, sound etc.)
    \item timed group discussions where one participant had to act on a certain prompt (e.g. \textit{try to encourage the person on your left to talk more}) whilst subject to some modality constraint (e.g. \textit{no speaking}) %took a constraint and/or a prompt which the other group members had to try to identify whilst reflecting on how that impacted the group experience
    \item an adapted version of the above where participants had to `program a robot' (the robot being role played by the first - third authors across their allocated groups) by instructing us how to deliver on that prompt. While acting on these instructions, we made sure only to act out explicit instructions given, e.g. keeping a monotone voice and refraining from gaze or head movements unless instructed otherwise.
\end{itemize}

% Firstly, we played an adapted version of 'telephone game'~\footnote{https://en.wikipedia.org/wiki/Chinese\_whispers} where group members had to stand in a line, with the first person turning and whispering an emotion or feeling to the person behind. This person had to communicate this feeling/emotion to the person behind through movement, then that person turn and pass it on by facial expression, then the next person by sound, to see if the final person in the line could say what the original emotion was. Next, we undertook a group discussion activity, where students were gathered around a table and given a question to discuss for two minutes. One student volunteered to take a constraint and/or a prompt card. Constraints included e.g. XXX and prompts included e.g. YYY. Once the two minutes was up, students discussed whether they could figure out the constraint and what it `felt like' when that group member interacted with them. 

% \subsection{`Robot' Assistant Activities}
% In order to prompt the students to think about how we might design/program social robot behaviours, specifically drawing attention to the need to specify \textit{multimodal} behaviours, we replicated the 2 minute group discussion setup from the previous activity, but this time has a student volunteer to pick from a new set of prompt cards (including e.g. AAA) and act as a robot `programmer'. That student had to sit behind the assigned group researcher, the `robot', and whisper to them what to do in order to deliver on the prompt. The researchers made sure to only act out the explicit instructions given, e.g. being careful to keep a monotone voice, and only to move/look at the person being spoken to if told to do so.  

% \subsubsection{No Robot Group Activity 1}

Participants also undertook an exemplar group activity (\textit{`No Robot' Group Activity 1} see Figure~\ref{fig:study_overview}) as per the robot training setup shown in Figure~\ref{fig:training}, but with the robot removed. The two participants sitting in (what would be) the RC and GO positions were tasked with observing the group and writing down any notable moments where they thought a robot could have assisted the group (and how it could have done so). %Students were rotated through these positions.   

\subsubsection{Co-Design of the Robot Action Space} \label{sec:comethodlogyaction}
We undertook an iterative action design process. First, we asked participants to come up with specific phrases or non-verbal gestures. We will refer to these specific phrases and gestures as action instances. Within their groups, we then asked participants to group those instances into overall more abstract action classes (with the help of their assigned researcher). These abstract action classes formed their proposed robot actions which then were pitched to the whole room. This allowed us (participants plus researchers) to identify overlapping/similar action classes across the groups. % and to discuss more group-specific ideas to agree on one, 
After a discussion between the three different groups facilitated by the researchers, participants agreed on a final set of shared robot actions.  %We then implemented some examples of these actions into the robot architecture ready for the students to test in their first session with the robot (ahead of final action instance generation) on day 3.   

\subsubsection{System design and action execution}
%We used the NAO's software development kit (SDK), to implement the co-designed actions, ROS for communication and Unity for imp. 
We used a tablet, as depicted in Figure \ref{fig:tablet}, to display the co-designed abstract actions. On execution of an abstract action, the system chose randomly from the list of concrete action instances. Teenagers designed the concrete instances and agreed upon the abstract action names on the tablet as described in section \ref{sec:comethodlogyaction}. Further, teenagers could select whom the action should be targeted at, the group or a specific individual. 


% \begin{figure}[htbp]
% \centerline{\includegraphics{design_hex.png}}
% \caption{Action design sheets were designed to prompt multi-modality and also had space to specify the action's aim, target (i.e. group or specific individual) and any specific trigger(s). [TO BE REPLACED WITH REAL EXAMPLE(S)]}
% \label{fig:actiondesign}
% \end{figure}

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.9\linewidth]{figures/sortingactions.png}}
% \caption{Group members go through the action instances they've each come up with (using our action design template) [ref supplementary materials?] and sort them into action classes representing their proposed robot action space for pitching to the other groups.}
% \label{fig:sortingactions}
% \end{figure}

% \subsubsection{First Session with the Robot} After the initial class negotiation, particpants' undertook an initial group session with the robot system (which had been equipped with a few initial instances of each co-designed action class) as per the experimental setup in Figure~\ref{fig:training}.

\subsubsection{Refinement of co-designed actions}
 After we implemented the actions on the robot, we invited participants to test the behaviours in a first robot group working session as detailed in \ref{sec:groupworking}. A subsequent class discussion confirmed that there were no additional abstract actions required. After having the chance to work with the robot %and the exemplar actions based on the initial class negotiated action space, 
 we asked participants to create as many instances of these abstract actions as possible, using a multimodal action design template we designed to help facilitate this process (provided in SM). %We pointed out that we would not be able to implement full body movements because NAO would be fixed in the seated position as per Figure~\ref{fig:training}. 
Notably, we had initially intended to let each group create and utilise only their action instances to increase the feeling of the robot being designed by and personalised to their specific group. However, the students quickly identified that there would be much more variety in the robot's actions if all groups pooled their action instances. %, and all agreed that they would prefer to take this approach, so 
Subsequently, groups shared the same cumulative set of robot action instances when working with the robot. %As all groups agreed this was the better thing to do, we pursued this approach instead. As such, when teaching the robot during group interactions, pressing e.g. the XX button on the teaching tablet would result one of the action instances from the full set of instances created across all three participant groups.   



\subsubsection{Robot Group Working Sessions}\label{sec:groupworking}
%Training of and testing/working with the robot was conducted in an adjoining, separate room to the main classroom in which we conducted whole class activities and where those not currently working with the robot worked on complimenting activities. 
 %The RC is equivalent to the \textit{domain expert teacher} referred to in the LEADOR method~\cite{winkle2021leador} and ``teaches" the robot what to by using a tablet to ``tell" the robot when to do which action. 
As noted previously, the aim of these sessions was to observe how RC participants utilised the robot and the impact this had on the group (equivalent, therefore, to a multi-session HRI study). %and (ii) to collect training data (training examples being made up of each RC action choice combined with a vector listing the value of each input feature at the moment that action was selected) with which we could train an ML agent to produce autonomous robot behaviour. 
The RC role is equivalent to the \textit{domain expert teacher} referred to in the LEADOR method~\cite{winkle2021leador}, and ``teaches" the robot what to do by using a tablet to ``tell" the robot when to do which action. The GO role was designed to reflect the \textit{witness} role utilised by Björling and Rose~\cite{bjorlingExploringTeensRobot2020} when undertaking in-the-wild robot studies with teenagers. 

The setup was fixed as per Figure~\ref{fig:training}. Whilst 3 out of 5 group members were working on a discussion-based group activity, one group member was controlling the robot's actions. The final group member was observing the group to support subsequent reflections. Working with the robot was conducted in an adjoining, separate room to the main classroom. We conducted whole class activities and hosted complimenting summer school activities  in the main classroom for those not currently working with the robot.

For each robot group working session, the students were left to work primarily unsupervised once the task had been explained. 
Researchers were sat in the adjacent room and occasionally checked on the group via the door window without interrupting. Sessions were made up of 3x15 minute rotations, in between which participants took quick breaks to complete quick post-session evaluations and swap roles, rotating between being the RC, GO or a GM. The group activities used for these sessions included a number of in-house designed discussion based activities plus adaptations of publicly available activities (such as the MIT AI ethics curriculum~\footnote{An Ethics of Artificial Intelligence Curriculum for Middle School Students was created by Blakeley H. Payne with support from the MIT Media Lab Personal Robots Group, directed by Cynthia Breazeal}). %Full details (including all materials required for replication) are provided in the SM.%, and we hope these might prove valuable to other researchers looking for discussion-based group activities that allow investigation of group behaviours. 
\subsubsection{Post-session questionnaire} After each 15 minute robot group working session, participants were asked to fill a short questionnaire. The questionnaire asked to indicate how well the group worked together on a positive five-point smiley scale~\cite{hall2016five}. The second question offered a continuous scale from 0 to 100 to rate the usefulness of the robot in terms of supporting the group interaction.

%These sessions were designed to simultaneously represent (i) training sessions whereby the robot controller's job was to `teach' the robot what it should do to be the best possible group assistant and (ii) user study evaluation sessions whereby participants could reflect on the impact (or lack thereof) of the robot. The setup was fixed as per Figure~\ref{fig:training} such that whilst 3 out of 5 of group members were working on a discussion-based group activity, one group member was controlling the robot's actions and the final group member was observing the group (using a second tablet to toggle pre-identified group behaviour descriptors of interest such as \textit{everyone is taking part}, \textit{too quiet/ silence} and \textit{uncomfortable/awkward}). For each training session, once the task had been explained, the students were left to work primarily unsupervised (researchers were sat in the adjacent room, occasionally checking on the group via the door window without interrupting) for 3x15 minute rotations, in between which they took quick breaks to complete quick post-session evaluations and swap roles, rotating between being a group member, the robot controller or the group observer. The group activities used for these sessions included a number of in-house designed discussion based activities plus adaptations of publicly available activities (such as the MIT AI ethics curriculum~\footnote{An Ethics of Artificial Intelligence Curriculum for Middle School Students was created by Blakeley H. Payne with support from the MIT Media Lab Personal Robots Group, directed by Cynthia Breazeal}). Full details (and links to materials for replication) are provided in the supplementary materials, and we hope these might prove valuable to other researchers looking for discussion-based group activities that allow investigation of group behaviours. 

\begin{figure}[tbp]
\input{figures/tablet_replace}
\caption{Tablet interface participants' used to control the robot (utilising the co-designed action space) during group activity sessions. Users' had to select the desired action and could identify an individual target GM where appropriate. Selecting an action only (with no individual target) resulted in an instance of the group-targeting version of that action.} %Note that with regards to the action-space implementation (and data collection regarding its use) the \textit{prompt discussion} action was subsumed into the \textit{ask opinion} action, as it essentially represented an \textit{ask opinion} action targeting the group (Table~\ref{tab:actionspace}).}
\label{fig:tablet}
\end{figure}

The data used for analyzing the use of the different actions was collected directly from the system. The system automatically noted which action was executed from the tablet, addressed towards whom. Further, we noted who was RC in each of the sessions. RCs indicated the specific seating position at the beginning of each session through the tablet. This information allowed us to analyze how different RCs controlled the robot. Further, we analyzed the actions that were targeted to specific individual GMs.

\subsection{Findings}\label{sec:codesign_findings}

%\subsection{How exactly could/should a group assistant robot behave in order to improve the group experience?}
The three key functions \textit{prompting discussion}, \textit{turn taking} and \textit{improving efficiency/performance} suggested in \ref{sec:focus_findings_use} %regarding how the robot might improve group working 
are reflected in the actions participants designed and refined for NAO during our iterative co-design process (Table~\ref{tab:actionspace}).´

%Whilst not raised specifically during the initial discussions, during individual action design participants created a number of actions centered around promoting the group (or specific individuals within the group) to stay focused in working towards task completion (see the Focus action in Table~\ref{tab:actionspace}), which we suggest also falls into this category of using the robot to improve efficiency/performance. 
Further, the use of the robot for improving efficiency and performance was reflected in the design. Participants created a different action centred around promoting the group (or specific individuals within the group) to stay focused in working towards task completion (see the Focus action in Table~\ref{tab:actionspace}). %, which we suggest also falls into this category of using the robot to improve efficiency/performance. 
%Table~\ref{tab:actionspace} identifies the robot actions resulting from our iterative co-designing process. 
Moreover, participants quickly identified after the initial tests that the robot should always refer to an individual by name when delivering an individual-targeted action in addition to looking at them.
% After initial testing of the robot on Day 3, participants quickly identified that, when delivering an individual-targeted action, the robot should always refer to that individual by name. 
This design choice had not initially been specified in any of the action instances they had created, seemingly becoming clear only upon working with the robot directly. We therefore appended target name in every (speech-based) individual-targeting action instance (see examples in Table~\ref{tab:actionspace}) during the action refinement phase. 
%After initial testing of the robot on Day 3, participants quickly identified that, when delivering an individual-targeted action, the robot should always refer to that individual by name. This was not something that was initially specified in any of the action instances they had created, but based on that feedback we included target name in every (speech-based) individual-targeting action instance (see examples in Table~\ref{tab:actionspace}). 

\begin{table}[]
\caption{Final co-designed action space of the group assistant robot. Actions default targeted the entire group unless the robot controller indicated a specific individual target via the teaching tablet (Figure \ref{fig:tablet}).}
\begin{center}
% \resizebox{\linewidth}{!}{
\begin{tabular}{|p{1cm}|p{1.2cm}|p{5cm}|}
\hline
Action                     & Target     & Example Speech (written by participants) \\ \hline
{Ask Opinion}       & Group      & Let's discuss our opinion about this! \\ \cline{2-3} 
%"Let's discuss our opinion about this! (group)
                          & Ind. & Do you have an opinion on this matter [name]? \\ \hline
 %Do you have an opinion on this matter [Group member]? 
{Agree}     & Group      & I agree.  \\ \cline{2-3} 
%"I agree."
                          & Ind. & I agree with you [name] \\ \hline
% "I agree with you [Group member]"
{Focus}     & Group      & Please can we stay focused on the activity? \\ \cline{2-3} 
% "Please can we stay focused on the activity?."
                          & Ind. & Don't forget the task [name]! \\ \hline
% "Don't forget the task!."
{Disagree}  & Group      & I don't agree with this. \\ \cline{2-3} 
%"I don't agree with this.
                          & Ind. & I don't agree with you [name] \\ \hline
% "I don't agree with you [GroupMember]"
{Joke}      & Group/Ind  & I wrote a song about a tortilla. Actually, it's more of a wrap! \\ \hline
%I wrote a song of a tortilla. Actually, it's more of a wrap!"  (same for both)                 
{Praise}    & Group      & Great job everyone! \\ \cline{2-3} 
%"Great job everyone!"
                          & Ind. & "Wow! Good thing you brought that up [name]!" \\ \hline
% "Wow! Good thing you brought that up!"
{Nod}       & Group/Ind    & - \\ \hline
{Elaborate} & Group      &  Really? Why do you think so? \\ \cline{2-3}
%Really? Why do you think so?"
                          & Ind. & Can you maybe explain more what you mean [name]? \\ \hline
% Can you maybe explain more what you mean [GroupMember]? 
{Look At}   & Group/Ind.      &  - \\ \hline
{Reminder}  & Group      & Remember: teamwork divides the task and multiplies the success. \\ \cline{2-3} 
%"remember: teamwork divides the task and multiplies the success."
                          & Ind. & [Name] remember that we are a team, we have to cooperate. \\ \hline
% "[GroupMember] remember that we are a team, we have to cooperate"                         
\end{tabular}
% }
\end{center}
\label{tab:actionspace}
\end{table}

%\subsection{Group - Robot Interactions}

%When operating the robot during robot training sessioIn conns, 
Different RCs utilised this common action space during robot training sessions with great variation between groups, seemingly reflecting that the groups were quite different and distinct in the way they interacted with each other. %and these differences appear to be reflected in the way Robot Controller's utilised the robot action space during the robot training sessions. 
%  reflects observed differences in how those groups behaved together and how therefore the robot could help best. For example, the \textit{Focus} action was used much more in the Baymax group (a group that appeared to struggle with maintaining task engagement) compared to R2D2 (a group that worked very well together) who instead appeared to use the robot as a mechanism for injecting some fun (via the \textit{Disagree} action) into their group work.
For instance, as can be seen in Fig.~\ref{fig:actionsgroups}, RCs in the Baymax group appeared to be using the robot in a teacher-like manner: prompting team members to focus on the required task and nudging them toward cooperation. %thus playing the role of a leader or teacher (used for authority/control). 
The R2D2 group, who appeared (and self-identified as being) more disciplined and capable of self-managing their teamwork, seemingly used the robot instead in a peer-like manner, using it more like a source of fun and entertainment. %As well as responding to (overall) group dynamics, Robot Controllers also seem to have responded to individual group members' personalities in their execution of individual-targeted actions. 

 %individual personalities. %to respond to individual group members' personalities whilst ing their individual personality. % but also seem as response to the personality of the recipient of individual-targeted actions.Robot Controllers within groups seem to have responded to individual group members' personalities in their execution of individual-targeted actions. 

%Within groups, we observed that the actions chosen by the Robot Controller reflected the controller's individual personality but also the personality of the recipient of individual-targeted actions. %Further, their action choices appear to somewhat reflect their own personalities.
%Within groups, we observed participants individual personalities being reflected in (a) the action choices they made when taking the Robot Controller role and (b) the actions targeted towards them by other Robot Controllers. %Further, their action choices appear to somewhat reflect their own personalities.
As well as responding to the current interaction in the group, RCs' action choices seemingly reflect their personalities and those of GM(s) their action choices target. For example, Figure~\ref{fig:P2P4} shows the actions %executed by, and 
targeted toward two participants within the Wall-E group. % in the %RC and 
%GM roles. % respectively. % at the actions used while training and received while being a group member by participants W2 and W4 in the Wall-E group, we can appreciate how different personalities/attitudes need, and at the same time model, different robot assistants profiles.
 %mainly used implicit modes of communication (\textit{look at, nod}) and rarely used more controlling or authoritarian actions (\textit{ask, focus, reminder} etc.). When in the GM role, 
The actions addressed towards W2 (self-identified introvert, often observed struggling to take part in the conversation) by the RCs seemingly tried to increase her engagement as they asked for her opinion or looked to her to elaborate more on ideas/opinions.
%When in the RC role, W2 (self-identified introvert, often observed struggling to take part in the conversation) mainly used implicit modes of communication (\textit{look at, nod}) and rarely used more controlling or authoritarian actions (\textit{ask, focus, reminder} etc.). When in the GM role, the actions addressed to her by the RCs seemingly tried to increase her engagement as they asked for her opinion or looked to her to elaborate more on ideas/opinions.

In contrast, W4 (self-identified extrovert, observed to be more often leading group discussions) received a wider variety of actions. Especially, W4 received those that might be considered indicative of greater (unprompted) participation but also perhaps an inclination to engage in off-topic discussions or become distracted/over-excited (i.e. \textit{agree, disagree, focus} and \textit{praise}). 
%Similarly when acting as the RC, W4 demonstrated great variety in his use of the action space, often making use of the \textit{joke} action as well as the \textit{ask} and \textit{focus} actions.

% \begin{figure}[t]
% \centerline{\includegraphics[width=0.45\linewidth]{figures/P2P4R_NEW.png}}
% \centerline{\includegraphics[width=0.45\linewidth]{figures/P2P4T_NEW.png}}
% \caption{Use of the robot's action space by two very different participants when acting as the Robot Controller, versus the actions that other Robot Controllers targeted towards them; with both seemingly reflecting those participants' different personalities (extroverted W4 versus introverted W2).}
% \label{fig:P2P4}
% \end{figure}

\begin{figure}[t]
\centerline{\includegraphics[height=4.5cm]{figures/actionbygroupNEW.png}}
\caption{Use of the robot's actions across the groups. The use of actions seemingly reflects  reflects observed differences in how those groups behaved together and how therefore the robot could help best. %For example, the \textit{Focus} action was used much more in the Baymax group (a group that appeared to struggle with maintaining task engagement) compared to R2D2 (a group that worked very well together) who instead appeared to use the robot as a mechanism for injecting some fun (via the \textit{Disagree} action) into their group work. 
Best viewed in color.}
\label{fig:actionsgroups}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[height=4.5cm]{figures/P2P4R_NEW.png}
    \caption{Use of the robot's action space towards two very different participants (extroverted W4 versus introverted W2). The received actions seemingly reflect their different personalities. Best viewed in color.}
    \label{fig:sfig1}
\end{figure}
% \begin{figure*}[t]
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.8\linewidth]{figures/P2P4R_NEW.png}
% %   \caption{...}
%   \label{fig:sfig1}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.8\linewidth]{figures/P2P4T_NEW.png}
% %   \caption{...}
%   \label{fig:sfig2}
% \end{subfigure}
\caption{Use of the robot's action space by two very different participants (extroverted W4 versus introverted W2) when acting as the RC, versus the actions that other RCs targeted towards them; with both seemingly reflecting their different personalities. Best viewed in color.}
\label{fig:P2P4}
\end{figure*}




%This leads us to think that the training of the robot was consciously done by the teenagers and that often, as pointed out in the focus groups, the preference for a co-design approach stems from the need to understand and engage with a group of peers from their unique perspective (they don't need a robot who is a teacher but a peer who can be authoritative when needed but also a cool guy.)
%All these observations lead us to reflect also on the importance of personalisation/adaptation of the robot?

% \begin{itemize}
%     \item did different kids use the actions space differently, i.e. using it to make fun (disagree) versus using it for authority/control (disagree); can we see reflections of the kids personalities/desire for the group in the robot like B4 vs B2 'serious' vs not? 
%     \item evaluations/experimental measures
%     \item I think here we should add some little group observations/reflections too to better contextualise our results, like it's imoportant to know that R2D2 was generally 'well behaved' task focused in a way that Baymax was less maybe in order to understand the focus group discussions (e.g. completely understandable why R2D2 would think the robot is having less impact than in Baymax) would be great if we can find some professional language (from the groups. literature maybe?) for words we use to properly describe them?
% \end{itemize}

% \subsection{Group Member Evaluations and Robot Controller Reflections}
% \begin{itemize}
%     \item something similar to table ~\ref{tab:norobotsessions} highlighting that the kids were generally pretty thoughtful in how they tried to use the action space; and simultaneously what the kids commented re. working with the robot
% \end{itemize}

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.9\linewidth]{actionstime.png}}
% \caption{Use of the robot's action space was fairly consistent as the summer school progressed; note that these four days represent a total of 8 distinct group-robot sessions.}
% \label{fig:actionstime}
% \end{figure}

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.9\linewidth]{figures/totalactions.png}}
% \centerline{\includegraphics[width=0.9\linewidth]{figures/specificaction.png}}
% \caption{The total number of actions targeted at individuals versus the group was quite similar, but specific actions were more often used in one form or the other (i.e. typically targeting an individual or the group) with the exception of the \textit{praise} action which was used fairly equally in both ways.}
% \label{fig:totalactionswho}
% \end{figure}

%\subsection{Day 8: Reflections on Working with the Robot}

==> sections/methodology.tex <==
\section{Design Methodologies}

Our overall approach was fundamentally centred around empowering students to lead in the co-design of a peer-designed robot group assistant. To this end, we refrained from specifying what our proposed group assistant robot should be trying to achieve beyond making group working \textit{`better'}; i.e. we left it to participants to tell us what `good' versus `bad' group working looked and felt like, how group working could be made better and what role, if any, a social robot might play in achieving this. We supported participants to do this by pursuing mutual learning processes, i.e. in Focus Group 1, after naive discussions on participants first thoughts, we conducted a researcher-led presentation designed to ensure participants had a realistic idea of social robot capabilities before re-opening discussions again. %~\cite{winkle2020mutual}) 
We also undertook a number of reflective group communication activities and games to get participants thinking about (multimodal) behaviours and the impact these can have on group members. These activities are discussed briefly below, but full details and related resources are provided in the supporting materials. We hope these might be useful for other researchers interested in group (robot) interactions. %Whilst initial co-design discussions and activities were robot-platform independent, we pre-selected the NAO robot as our robot of choice for specific action co-design and test.  

% [what design brief did we set the students re. the role of the robot (links to the focus groups, we obviously explained the type of activities thye'd be doing as they experienced in the no robot activity but did not set any specifics regarding whayt *we* thought a good robot/group should look like e.g. it's about balancing participation, only what they believe 'better' groups would look like as they had discussed and identified during the focus groups]

% we will make all of our own materials (design sheets, slides, game instructions, topic guides etc.) publicly available for other researchers --> perhaps include them as supplementary material with the paper
% covered
\subsection{Focus Groups and Interviews}
As noted in Table~\ref{tab:timetable} we utilised focus groups and interviews at four key stages of the programme:
\begin{itemize}
\item[(i)] \textit{Focus Group 1 - Application of the Robot}: capturing teenagers' expert knowledge with respect to groups and exploring initial ideas of how social robots could support and improve group working; supported by an interim researcher-led presentation introducing some example robots/applications from related literature to support mutual learning~\cite{winkle2020mutual}. 
\item[(ii)] \textit{Focus Group 2 - Reflection on the Robot and its Impact}: re-visiting some of the topics from Day 1 now informed by the experience of the robot, i.e. what (if any) impact the robot had during group working. Also included reflection on the robot teaching experience and RC-GM-GO setup.
\item[(iii)] \textit{Group Interview - Removing the Robot}: a quick interview with participants towards the end of the summer school, after they undertook a group activity without the robot being present. 
\item[(iv)] \textit{Group Interview - Testing the Autonomous Robot}: a quick interview with participants after they undertook a group activity with a first autonomous version of the robot, created by application of ML to the training data collected during the the robot `training sessions'.
\end{itemize}

The topic guides for the more structured Focus Groups 1 and 2 are provided in the supplementary materials. %Note we specifically followed mutual shaping methodology in Focus Group 1 with discussions taking place pre- and post- a researcher-led presentation on related HRI literature to capture participants' naive and unbiased ideas with respect to what role the robot should take~\cite{winkle2020mutual}. 
Resultant data were coded for key results following the Framework Method~\cite{ritchie2013qualitative} i.e., using a combined deductive and inductive approach to coding but primarily guided by the latter, with only a couple of high level initial codes being generated according to the research questions. Three of the authors then independently coded the data collected from the participant group they had worked with most, generating data-driven inductive codes as required. The results were discussed and a final coding scheme was generated for application to all data. 

% \subsubsection{Group Debrief 2 - Post-Turing Test}
% on ... [implementation details]

% \begin{table}[]
% \begin{center}
% \caption{...}
% \begin{tabular}{|l|l|}
% \hline
% Session                                                                              & Topic Guide                                                                        \\ \hline
% \begin{tabular}[c]{@{}l@{}}Day 1 Focus Group\\ (Robots and Groups)\end{tabular}      & \begin{tabular}[c]{@{}l@{}}...\\ {[}Break: Researcher Presentation{]}\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Day 8 Focus Group\\ (Robots and Groups)\end{tabular}      & \begin{tabular}[c]{@{}l@{}}...\\ ...\\ ...\end{tabular}                            \\ \hline
% \begin{tabular}[c]{@{}l@{}}Day 9 Group Interview\\ (Removing the Robot)\end{tabular} & \begin{tabular}[c]{@{}l@{}}...\\ ...\\ ...\end{tabular}                            \\ \hline
% \end{tabular}
% \label{tab:topicguides}
% \end{center}
% \end{table}

\subsection{Group Communication and `Robot' Assistant Activities and Games}
Ahead of starting detailed action space co-design we undertook a number of reflective activities to first get participants thinking about multimodal communication in groups; specifically how one member's behaviours can influence the group experience, and how robots might need to be explicitly programmed to do e.g. nonverbal behaviours we often take for granted. %In order to prompt the students to think (specifically multimodal) behaviour in groups, we undertook a number of group, game-like activities whereby they had to reflect on their own and/or the group's behaviour. 
These included:
\begin{itemize}
    \item an adapted version of the `telephone game'~\footnote{\url{https://en.wikipedia.org/wiki/Chinese_whispers}} where participants had to pass a message between themselves with each person using a different modality (movement, facial expression, sound etc.)
    \item timed group discussions where one participant had to act on a certain prompt (e.g. \textit{try to encourage the person on your left to talk more}) whilst subject to some modality constraint (e.g. \textit{no speaking}) %took a constraint and/or a prompt which the other group members had to try to identify whilst reflecting on how that impacted the group experience
    \item an adapted version of the above where participants had to `program a robot' (the robot being roleplayed by the first - third authors across their allocated groups) by instructing us how to deliver on that prompt, whilst we made sure to only act out explicit instructions given e.g. keeping a monotone voice and refraining from gaze or head movements unless instructed otherwise.
\end{itemize}

% Firstly, we played an adapted version of 'telephone game'~\footnote{https://en.wikipedia.org/wiki/Chinese\_whispers} where group members had to stand in a line, with the first person turning and whispering an emotion or feeling to the person behind. This person had to communicate this feeling/emotion to the person behind through movement, then that person turn and pass it on by facial expression, then the next person by sound, to see if the final person in the line could say what the original emotion was. Next, we undertook a group discussion activity, where students were gathered around a table and given a question to discuss for two minutes. One student volunteered to take a constraint and/or a prompt card. Constraints included e.g. XXX and prompts included e.g. YYY. Once the two minutes was up, students discussed whether they could figure out the constraint and what it `felt like' when that group member interacted with them. 

% \subsection{`Robot' Assistant Activities}
% In order to prompt the students to think about how we might design/program social robot behaviours, specifically drawing attention to the need to specify \textit{multimodal} behaviours, we replicated the 2 minute group discussion setup from the previous activity, but this time has a student volunteer to pick from a new set of prompt cards (including e.g. AAA) and act as a robot `programmer'. That student had to sit behind the assigned group researcher, the `robot', and whisper to them what to do in order to deliver on the prompt. The researchers made sure to only act out the explicit instructions given, e.g. being careful to keep a monotone voice, and only to move/look at the person being spoken to if told to do so.  

% \subsubsection{No Robot Group Activity 1}

Participants also undertook an exemplar group activity (\textit{`No Robot' Group Activity 1} per Table~\ref{tab:timetable}) as per the robot training setup shown in Figure~\ref{fig:training}, but with the robot removed. The two participants sitting in (what would be) the RC and GO positions were tasked with observing the group and writing down any notable moments where they thought a robot could have assisted the group (and how it could have done so). %Students were rotated through these positions.   

\subsection{Co-Design of the Robot Action Space}
We undertook an iterative action design process, first asking participants to come up with specific action instances and then, within their groups, to group those instances into overall action classes (with the help of their assigned researcher) to make up their proposed robot action space. Groups then pitched their action spaces to the whole room such that together we (participants plus researchers) identified overlapping/similar action classes across the groups and discussing more group-specific ideas to agree on one, final shared robot action space. We then implemented some examples of these actions into the robot architecture ready for the students to test in their first session with the robot (ahead of final action instance generation) on day 3.   

% \begin{figure}[htbp]
% \centerline{\includegraphics{design_hex.png}}
% \caption{Action design sheets were designed to prompt multi-modality and also had space to specify the action's aim, target (i.e. group or specific individual) and any specific trigger(s). [TO BE REPLACED WITH REAL EXAMPLE(S)]}
% \label{fig:actiondesign}
% \end{figure}

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.9\linewidth]{figures/sortingactions.png}}
% \caption{Group members go through the action instances they've each come up with (using our action design template) [ref supplementary materials?] and sort them into action classes representing their proposed robot action space for pitching to the other groups.}
% \label{fig:sortingactions}
% \end{figure}

% \subsubsection{First Session with the Robot} After the initial class negotiation, particpants' undertook an initial group session with the robot system (which had been equipped with a few initial instances of each co-designed action class) as per the experimental setup in Figure~\ref{fig:training}.

%\subsubsection{Final Instance Generation}
A subsequent class discussion confirmed there were no additional actions required. After having chance to work with the robot and the exemplar actions based on the initial class negotiated action space, participants were asked to come up with as many instances of these actions as possible, using a multimodal action design template we designed to help facilitate this process (provided in SM). %We pointed out that we would not be able to implement full body movements because NAO would be fixed in the seated position as per Figure~\ref{fig:training}. 
Notably, we had originally intended to let each group create and utilise only their own action instances to increase the feeling of the robot being designed by, and personalised to, their specific group. However, the students quickly identified there would be much more variety in the robot's actions if all groups pooled their action instances, and all agreed that they would prefer to take this approach, so groups shared the same cumulative set of robot action instances when it came to working with the robot. %As all groups agreed this was the better thing to do, we pursued this approach instead. As such, when teaching the robot during group interactions, pressing e.g. the XX button on the teaching tablet would result one of the action instances from the full set of instances created across all three participant groups.   

\subsection{Robot Activity Training Sessions}
%Training of and testing/working with the robot was conducted in an adjoining, separate room to the main classroom in which we conducted whole class activities and where those not currently working with the robot worked on complimenting activities. 
 %The RC is equivalent to the \textit{domain expert teacher} referred to in the LEADOR method~\cite{winkle2021leador} and ``teaches" the robot what to by using a tablet to ``tell" the robot when to do which action. 
As noted previously, the aim of these sessions were to (i) observe how RC participants utilised the robot and the impact this had on the group (equivalent therefore to a multi-session HRI study) and (ii) to collect training data (training examples being made up of each RC action choice combined with a vector listing the value of each input feature at the moment that action was selected) with which we could train an ML agent to produce autonomous robot behaviour. The RC role is equivalent to the \textit{domain expert teacher} referred to in the LEADOR method~\cite{winkle2021leador} and ``teaches" the robot what to do by using a tablet to ``tell" the robot when to do which action. The GO role was designed to reflect the \textit{witness} role utilised by Björling and Rose~\cite{bjorlingExploringTeensRobot2020} when undertaking in-the-wild robot studies with teenagers. 

The setup was fixed as per Figure~\ref{fig:training} such that whilst 3 out of 5 of group members were working on a discussion-based group activity, one group member was controlling the robot's actions and the final group member was observing the group (using a second tablet to toggle group behaviour descriptors identified as being relevant during Focus Group 1 e.g. \textit{everyone is taking part}, \textit{too quiet/ silence} and \textit{uncomfortable/awkward}). Training of and testing/working with the robot was conducted in an adjoining, separate room to the main classroom in which we conducted whole class activities and hosted complimenting summer school activities for those not currently working with the robot.

For each training session, once the task had been explained, the students were left to work primarily unsupervised - researchers were sat in the adjacent room, occasionally checking on the group via the door window without interrupting. Sessions were made up of 3x15 minute rotations, in between which participants took quick breaks to complete quick post-session evaluations and swap roles, rotating between being the RC, GO or a GM. The group activities used for these sessions included a number of in-house designed discussion based activities plus adaptations of publicly available activities (such as the MIT AI ethics curriculum~\footnote{An Ethics of Artificial Intelligence Curriculum for Middle School Students was created by Blakeley H. Payne with support from the MIT Media Lab Personal Robots Group, directed by Cynthia Breazeal}). Full details (including all materials required for replication) are provided in the SM.%, and we hope these might prove valuable to other researchers looking for discussion-based group activities that allow investigation of group behaviours. 

%These sessions were designed to simultaneously represent (i) training sessions whereby the robot controller's job was to `teach' the robot what it should do to be the best possible group assistant and (ii) user study evaluation sessions whereby participants could reflect on the impact (or lack thereof) of the robot. The setup was fixed as per Figure~\ref{fig:training} such that whilst 3 out of 5 of group members were working on a discussion-based group activity, one group member was controlling the robot's actions and the final group member was observing the group (using a second tablet to toggle pre-identified group behaviour descriptors of interest such as \textit{everyone is taking part}, \textit{too quiet/ silence} and \textit{uncomfortable/awkward}). For each training session, once the task had been explained, the students were left to work primarily unsupervised (researchers were sat in the adjacent room, occasionally checking on the group via the door window without interrupting) for 3x15 minute rotations, in between which they took quick breaks to complete quick post-session evaluations and swap roles, rotating between being a group member, the robot controller or the group observer. The group activities used for these sessions included a number of in-house designed discussion based activities plus adaptations of publicly available activities (such as the MIT AI ethics curriculum~\footnote{An Ethics of Artificial Intelligence Curriculum for Middle School Students was created by Blakeley H. Payne with support from the MIT Media Lab Personal Robots Group, directed by Cynthia Breazeal}). Full details (and links to materials for replication) are provided in the supplementary materials, and we hope these might prove valuable to other researchers looking for discussion-based group activities that allow investigation of group behaviours. 

\begin{figure}[tbp]
\input{figures/tablet_replace}
\caption{Tablet interface participants' used to control the robot (utilising the co-designed action space) during group activity sessions. Users' had to select the desired action and could identify an individual target GM where appropriate. Selecting an action only (with no individual target) resulted in an instance of the group-targeting version of that action.} %Note that with regards to the action-space implementation (and data collection regarding its use) the \textit{prompt discussion} action was subsumed into the \textit{ask opinion} action, as it essentially represented an \textit{ask opinion} action targeting the group (Table~\ref{tab:actionspace}).}
\label{fig:tablet}
\end{figure}


% \subsection{Experimental Measures}
% We After each 15x minute activity session, all group members completed a quick questionnaire specific to their role during the session. Questionnaire items are given in Table~\ref{tab:expquest}. We recorded all actions executed on the robot by the Robot Controllers as well as...[what else to list here, everything or only what we present/refer to in the paper?]. 

% \begin{table}[]
% \caption{Quick survey measures participants completed after each 15 minute group/robot activity session. Full measures (as they were provided to the students) are provided in the supplementary materials.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|l|l|l|}
% \hline
% Questionnaire Item                                                                                                                                         & Answer Type   & Group Role(s)                                                                           \\ \hline
% How much did you enjoy the activity?                                                                                                                       & Emoji Likert  & Group Member                                                                            \\ \hline
% \begin{tabular}[c]{@{}l@{}}We all liked the way we worked \\ together.\end{tabular}                                                                        & Emoji Likert  & Group Member                                                                            \\ \hline
% \begin{tabular}[c]{@{}l@{}}Can you give some more details? How\\ was the activity, how well do you feel \\ the group worked together and why?\end{tabular} & Free text     & Group Member                                                                            \\ \hline
% \begin{tabular}[c]{@{}l@{}}Everyone in the group seemed to like \\ the way they worked together.\end{tabular}                                              & Emoji Likert  & \begin{tabular}[c]{@{}l@{}}Group Observer\\ Robot Controller\end{tabular}               \\ \hline
% \begin{tabular}[c]{@{}l@{}}Can you explain more? What did you\\  observe?\end{tabular}                                                                     & Free text     & Group Observer                                                                          \\ \hline
% \begin{tabular}[c]{@{}l@{}}I think the robot helped the group work \\ well together.\end{tabular}                                                          & 0 - 100 Scale & \begin{tabular}[c]{@{}l@{}}Group Member\\ Group Observer\\ Robot Conroller\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Can you describe any specific moments \\ where the robot seemed to have an \\ impact on the group (good or bad)?\end{tabular}   & Free text     & \begin{tabular}[c]{@{}l@{}}Group Member\\ Group Observer\end{tabular}                   \\ \hline
% \begin{tabular}[c]{@{}l@{}}How did you try to have the robot assist\\  the group?  Do you think it worked?\end{tabular}                                    & Free text     & Robot Controller                                                                        \\ \hline
% \end{tabular}}
% \label{tab:expquest}
% \end{table}

% [surveys]
% [audio/other automatic/'objective' measures i.e. speaker participation and balance?]
% For the purposes of informing group robot design guidelines, we also consider students' action choices and group observation labels (all automatically recorded by our system) to also represent pertinent experimental results, particularly when combined with the student evaluations. 

% \section{A Corpus of Group Robot Co-Design and Test Activities}
% [maybe a comment here about all the activities we came up with hopefully being useful to other researchers, esp. if we share them all as supplementary materials]

% \begin{table}[]
% \caption{Overview of the discussion based group activities undertaken with/without the robot for testing, training and evaluation.}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Activity\\ (n sessions)\end{tabular}             & Description \\ \hline
% \begin{tabular}[c]{@{}l@{}}Designing Furhat\\ (x sessions)\end{tabular}     &             \\ \hline
% \begin{tabular}[c]{@{}l@{}}Smart Your City\\ (x sessions)\end{tabular}      &             \\ \hline
% \begin{tabular}[c]{@{}l@{}}Interviewing Cozmo\\ (x sessions)\end{tabular}   &             \\ \hline
% \begin{tabular}[c]{@{}l@{}}Re-Designing Youtube\\ (x sessions)\end{tabular} &  Adapted from the MIT AI Ethics Curriculum\footnote{An Ethics of Artificial
% Intelligence Curriculum for Middle School Students was created by Blakeley
% H. Payne with support from the MIT Media Lab Personal Robots Group,
% directed by Cynthia Breazeal.}           \\ \hline
% \begin{tabular}[c]{@{}l@{}}Speculative Futures\\ (x sessions)\end{tabular}  &  Adapted from the MIT AI Ethics Curriculum           \\ \hline
% \begin{tabular}[c]{@{}l@{}}Which Robot?\\ (x sessions)\end{tabular}         &             \\ \hline
% \begin{tabular}[c]{@{}l@{}}The Empathy Robot\\ (x sessions)\end{tabular}    &             \\ \hline
% \begin{tabular}[c]{@{}l@{}}A Robot Story\\ (x sessions)\end{tabular}        &             \\ \hline
% \end{tabular}}
% \label{tab:trainingactivities}
% \end{table}


% \section{Findings}
% \label{sec:results}

% \subsection{Teen Groups}

%\subsection{Day 1: Robots for Groups}

==> sections/results_rq1.tex <==
\section{Teen Design and Use of a Group Assistant Robot (RQ1)}
% \begin{itemize}
%     \item robot to ask questions and prompt discussion; ice breaking for everyone + comments around turntaking but some skepticim (in R2D2 specifically) about need/impact for robots if you already know the group
%     \item comments on improving efficiency
% \end{itemize}
\subsection{(How) do teens envisage robots being able to improve their groups?}
%\newline 
Initial ideas on how a robot might help to improve their groups broadly fell into three categories: \textit{prompting discussion}, \textit{turn taking} and \textit{improving efficiency/performance}. On \textit{prompting discussion}, all groups identified the potential for a robot to act as an ice-breaker and to ease awkwardness: \textit{``It's mostly about starting that conversation and then it'll take on and then everyone else will start talking"} (W2).
% \textit{``And they could be like how you do it, or in math. It's like it's a group. They're like, OK, let's get started like they talk for us.''} (W4)
% \textit{``Maybe like choosing between speaking next. This is why because probably no ones wants to speak first like so maybe the robot can help everyone to take the turn."} (B1)  
But more specifically on turn-taking, participants also referred to making sure everyone got to speak, and/or perhaps encouraging those who were quiet: \textit{``It starts and then if someone talks way too much it like: sh sh sh, let this one talk"} (W3).
% \textit{``When I get silent, ask another question or something.''} (W2)
% \textit{The robot could like act like, maybe that they like don't understand. So it will say like can you explain so then you'll have to talk and maybe that will make other people add stuff.} (R2).

However there was some hesitation in the R2D2 group as to whether that was really necessary/helpful in groups that already know each other: \textit{``When you don't know anyone that I think maybe robots can be like good at like organising and making sure that everyone can talk... I feel like if you know the people you are in a group with it I feel like it would more be like the group and the robot, not like the robot helping the group"} (R2).

On \textit{improving efficiency/performance} ideas a common theme centered on how the robot could help with the task by answering questions or acting as an interface to the internet: \textit{``Like a computer, it tells you the answers. You have to work on an assignment you have the robot that is like the computer or google, it can help you to find out the answer for your assignment''} (B4). Implementation of a (teen-safe) robot-internet interface was not feasible in our study timeframe so we were unable to support participants in creating actions relating to such a function, but we note it here for future works. Whilst not raised specifically during the initial discussions, during individual action design participants created a number of actions centered around promoting the group (or specific individuals within the group) to stay focused in working towards task completion (see the Focus action in Table~\ref{tab:actionspace}), which we suggest also falls into this category of using the robot to improve efficiency/performance. 

The researcher-led presentation highlighting related prior works~\cite{Shen2018, Tennent2019, Strohkorb2016,strohkorb2018ripple,Short2017Understanding} also seemed to strengthen participants' ideas on using a robot for turn-taking and, more specifically, to improve inclusiveness. \textit{Micbot}, a robot microphone which rotates in order to try and equalise speaking time and participation during group discussions~\cite{Tennent2019} was particularly well received (a favourite within R2D2 and Baymax) with participants being impressed at how simple yet effective it was at getting all group members to participate in the discussion: \textit{``Well, what I liked about the micbot...it gave everyone a voice. in a way that I think that I don't really feel like [keepon \cite{Shen2018}] could do. I don't know how they could do it in the same way"} (R1). This potential for the management of turn-taking to increase inclusiveness seemed to appeal equally to participants who self-identified as (and were observed to be) both more extroverted/confident and more introverted/shy: \textit{``And it's going to let the shy person be able to talk...and everyone after might not speak over him"} (W4, more extroverted); \textit{``I can't interrupt them and then I am screwed. So I wait and wait and wait. So this microphone will be really good so I could talk to the others"} (W2, more introverted).
%Initial feedback after the researcher-led presentation (which highlighted a selection of previous works on robots for groups~\cite{Shen2018, Tennent2019, Strohkorb2016,strohkorb2018ripple,Short2017Understanding} suggested \textit{micbot}~\cite{Tennent2019} was particularly well received (a favourite within R2D2 and Baymax) with participants being impressed at how simple yet effective it was at getting all group members to participate in the discussion: \textit{``Well, what I liked about the mic bot, I think it is because it was like a mic. Yeah it gave everyone a voice. in a way that I think that I don't really feel like [keepon] could do. I don't know how they could do it in the same way"} (R1).

% micbot for group participation~\cite{}, keepon for conflict resolution~\cite{}, xxx for intergenerational communication~\cite{} and NAO for yyy~\cite{})... suggested the micbot was particularly well received (a favourite within R2D2 and Baymax) with participants being impressed at how simple yet effective it was at getting all group members to participate in the discussion: %However, there were conflicting ideas as to whether it's simplistic appearance was a positive feature or a potential limitation.

% \textit{[Which was your favourite?] The microphone one? Because yeah, because it like tells it says who can talk and if it's one person that hasn't talked that much it like tells that person it's their time...make it like maybe look a bit more like [NAO]} (B2)



% \textit{``I love how like simple yet practical [micbot] is like of course the microphone should be able to rotate, but yeah, it was like smart... in work circumstances like you don't want a purple, a cute robot really.''} (R2)

%This also seemed to strengthen participants' ideas on using a robot for turn-taking and, more specifically, to improve inclusiveness, as these came up again on re-visiting potential robot applications after the presentation. 

%This also seemed to strengthen participants' ideas on using a robot for turn-taking and, more specifically, to improve inclusiveness, as these came up again on re-visiting potential robot applications after the presentation. Notably this seemed to appeal to students who self-identified as (and were later also observed to be) more extroverted/confident in group discussions or more introverted/struggling to speak sometimes: \textit{``And it's going to let the shy person be able to talk...and everyone after might not speak over him"} (W4); \textit{``I can't interrupt them and then I am screwed. So I wait and wait and wait. So this microphone will be really good so I could talk to the others"} (W2).

\subsection{How exactly could/should a group assistant robot behave in order to improve the group experience?}
The three key functions suggested above regarding how the robot might improve group working are clearly reflected in the robot actions participants designed and refined for NAO during our iterative co-design process (Table~\ref{tab:actionspace}). %Table~\ref{tab:actionspace} identifies the robot actions resulting from our iterative co-designing process. 
After initial testing of the robot on Day 3, participants quickly identified that the robot should always refer to an individual by name when delivering an individual-targeted action.
% After initial testing of the robot on Day 3, participants quickly identified that, when delivering an individual-targeted action, the robot should always refer to that individual by name. 
This had not initially been specified in any of the action instances they had created, seemingly becoming clear only upon working with the robot directly. We therefore post-hoc appended target name in every (speech-based) individual-targeting action instance (see examples in Table~\ref{tab:actionspace}) based on that feedback ahead of Day 4. 
%After initial testing of the robot on Day 3, participants quickly identified that, when delivering an individual-targeted action, the robot should always refer to that individual by name. This was not something that was initially specified in any of the action instances they had created, but based on that feedback we included target name in every (speech-based) individual-targeting action instance (see examples in Table~\ref{tab:actionspace}). 

\begin{table}[]
\caption{Final co-designed action space of the group assistant robot. Actions default targeted the entire group unless the robot controller indicated a specific individual target via the teaching tablet (Figure \ref{fig:tablet}).}
\begin{center}
% \resizebox{\linewidth}{!}{
\begin{tabular}{|p{1cm}|p{1.2cm}|p{5cm}|}
\hline
Action                     & Target     & Example Speech (written by participants) \\ \hline
{Ask Opinion}       & Group      & Let's discuss our opinion about this! \\ \cline{2-3} 
%"Let's discuss our opinion about this! (group)
                          & Ind. & Do you have an opinion on this matter [name]? \\ \hline
 %Do you have an opinion on this matter [Group member]? 
{Agree}     & Group      & I agree.  \\ \cline{2-3} 
%"I agree."
                          & Ind. & I agree with you [name] \\ \hline
% "I agree with you [Group member]"
{Focus}     & Group      & Please can we stay focused on the activity? \\ \cline{2-3} 
% "Please can we stay focused on the activity?."
                          & Ind. & Don't forget the task [name]! \\ \hline
% "Don't forget the task!."
{Disagree}  & Group      & I don't agree with this. \\ \cline{2-3} 
%"I don't agree with this.
                          & Ind. & I don't agree with you [name] \\ \hline
% "I don't agree with you [GroupMember]"
{Joke}      & Group/Ind  & I wrote a song about a tortilla. Actually, it's more of a wrap! \\ \hline
%I wrote a song of a tortilla. Actually, it's more of a wrap!"  (same for both)                 
{Praise}    & Group      & Great job everyone! \\ \cline{2-3} 
%"Great job everyone!"
                          & Ind. & "Wow! Good thing you brought that up [name]!" \\ \hline
% "Wow! Good thing you brought that up!"
{Nod}       & Group/Ind    & - \\ \hline
{Elaborate} & Group      &  Really? Why do you think so? \\ \cline{2-3}
%Really? Why do you think so?"
                          & Ind. & Can you maybe explain more what you mean [name]? \\ \hline
% Can you maybe explain more what you mean [GroupMember]? 
{Look At}   & Group/Ind.      &  - \\ \hline
{Reminder}  & Group      & Remember: teamwork divides the task and multiplies the success. \\ \cline{2-3} 
%"remember: teamwork divides the task and multiplies the success."
                          & Ind. & [Name] remember that we are a team, we have to cooperate. \\ \hline
% "[GroupMember] remember that we are a team, we have to cooperate"                         
\end{tabular}
% }
\end{center}
\label{tab:actionspace}
\end{table}

%\subsection{Group - Robot Interactions}

%When operating the robot during robot training sessions, 
The way that different RCs utilised this common action space during robot training session varied quite significantly between groups, seemingly reflecting that the groups were quite different and distinct in the way they interacted with each other. %and these differences appear to be reflected in the way Robot Controller's utilised the robot action space during the robot training sessions. 
For instance, as can be seen in Fig.~\ref{fig:actionsgroups}, RCs in the Baymax group appeared to be use the robot in a teacher-like manner: prompting team members to focus on the required task and nudging them towards cooperation. %thus playing the role of a leader or teacher (used for authority/control). 
The R2D2 group, who appeared (and self-identified as being) more  disciplined and capable of self-managing their teamwork, seemingly used the robot instead in a peer-like manner, using it more like a source of fun and entertainment. %As well as responding to (overall) group dynamics, Robot Controllers also seem to have responded to individual group members' personalities in their execution of individual-targeted actions. 

 %individual personalities. %to respond to individual group members' personalities whilst ing their individual personality. % but also seem as response to the personality of the recipient of individual-targeted actions.Robot Controllers within groups seem to have responded to individual group members' personalities in their execution of individual-targeted actions. 

%Within groups, we observed that the actions chosen by the Robot Controller reflected the controller's individual personality but also the personality of the recipient of individual-targeted actions. %Further, their action choices appear to somewhat reflect their own personalities.
%Within groups, we observed participants individual personalities being reflected in (a) the action choices they made when taking the Robot Controller role and (b) the actions targeted towards them by other Robot Controllers. %Further, their action choices appear to somewhat reflect their own personalities.
As well as responding to (overall) group dynamics, RCs' action choices seemingly reflect their own personalities as well as those of GM(s) their action choices target. For example, Figure~\ref{fig:P2P4} shows the actions executed by, and targeted towards, two participants within the Wall-E group when they were in the RC and GM roles respectively. % at the actions used while training and received while being a group member by participants W2 and W4 in the Wall-E group, we can appreciate how different personalities/attitudes need, and at the same time model, different robot assistants profiles.
When in the RC role, W2 (self-identified introvert, often observed struggling to take part in the conversation) mainly used implicit modes of communication (\textit{look at, nod}) and rarely used more controlling or authoritarian actions (\textit{ask, focus, reminder} etc.). When in the GM role, the actions addressed to her by the RCs seemingly tried to increase her engagement as they asked for her opinion or looked to her to elaborate more on ideas/opinions.

In contrast, W4 (self-identified extrovert, observed to be more often leading group discussions) received a larger variety of actions, especially those ones that might be considered indicative of greater (unprompted) participation but also perhaps an inclination to engage in off-topic discussions or become distracted/over-excited (i.e. \textit{agree, disagree, focus} and \textit{praise}, etc.). Similarly when acting as the RC, W4 demonstrated great variety in his use of the action space, often making use of the \textit{joke} action as well as the \textit{ask} and \textit{focus} actions.

% \begin{figure}[t]
% \centerline{\includegraphics[width=0.45\linewidth]{figures/P2P4R_NEW.png}}
% \centerline{\includegraphics[width=0.45\linewidth]{figures/P2P4T_NEW.png}}
% \caption{Use of the robot's action space by two very different participants when acting as the Robot Controller, versus the actions that other Robot Controllers targeted towards them; with both seemingly reflecting those participants' different personalities (extroverted W4 versus introverted W2).}
% \label{fig:P2P4}
% \end{figure}

\begin{figure}[t]
\centerline{\includegraphics[width=1\linewidth]{figures/actionbygroupNEW.png}}
\caption{Use of the robot's action space across the groups reflects observed differences in how those groups behaved together and how therefore the robot could help best. For example, the \textit{Focus} action was used much more in the Baymax group (a group that appeared to struggle with maintaining task engagement) compared to R2D2 (a group that worked very well together) who instead appeared to use the robot as a mechanism for injecting some fun (via the \textit{Disagree} action) into their group work.}
\label{fig:actionsgroups}
\end{figure}

\begin{figure*}[t]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/P2P4R_NEW.png}
%   \caption{...}
  \label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/P2P4T_NEW.png}
%   \caption{...}
  \label{fig:sfig2}
\end{subfigure}
\caption{Use of the robot's action space by two very different participants (extroverted W4 versus introverted W2) when acting as the RC, versus the actions that other RCs targeted towards them; with both seemingly reflecting their different personalities. Best viewed in color.}
\label{fig:P2P4}
\end{figure*}

%This leads us to think that the training of the robot was consciously done by the teenagers and that often, as pointed out in the focus groups, the preference for a co-design approach stems from the need to understand and engage with a group of peers from their unique perspective (they don't need a robot who is a teacher but a peer who can be authoritative when needed but also a cool guy.)
%All these observations lead us to reflect also on the importance of personalisation/adaptation of the robot?

% \begin{itemize}
%     \item did different kids use the actions space differently, i.e. using it to make fun (disagree) versus using it for authority/control (disagree); can we see reflections of the kids personalities/desire for the group in the robot like B4 vs B2 'serious' vs not? 
%     \item evaluations/experimental measures
%     \item I think here we should add some little group observations/reflections too to better contextualise our results, like it's imoportant to know that R2D2 was generally 'well behaved' task focused in a way that Baymax was less maybe in order to understand the focus group discussions (e.g. completely understandable why R2D2 would think the robot is having less impact than in Baymax) would be great if we can find some professional language (from the groups. literature maybe?) for words we use to properly describe them?
% \end{itemize}

% \subsection{Group Member Evaluations and Robot Controller Reflections}
% \begin{itemize}
%     \item something similar to table ~\ref{tab:norobotsessions} highlighting that the kids were generally pretty thoughtful in how they tried to use the action space; and simultaneously what the kids commented re. working with the robot
% \end{itemize}

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.9\linewidth]{actionstime.png}}
% \caption{Use of the robot's action space was fairly consistent as the summer school progressed; note that these four days represent a total of 8 distinct group-robot sessions.}
% \label{fig:actionstime}
% \end{figure}

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.9\linewidth]{figures/totalactions.png}}
% \centerline{\includegraphics[width=0.9\linewidth]{figures/specificaction.png}}
% \caption{The total number of actions targeted at individuals versus the group was quite similar, but specific actions were more often used in one form or the other (i.e. typically targeting an individual or the group) with the exception of the \textit{praise} action which was used fairly equally in both ways.}
% \label{fig:totalactionswho}
% \end{figure}

%\subsection{Day 8: Reflections on Working with the Robot}

==> sections/results_rq2.tex <==

\section{Group-Robot Dynamics and (Evolving) Impact of the Robot on Group Working (RQ2)}

Given the scarcity of child-robot interaction studies which extend beyond a single interaction (thus likely falling victim to the well known novelty effect~\cite{bartneck2020human}) we specifically examine how participants' reactions to and thoughts about the robot evolved over the course of our 2 week summer school, across which each group worked with the robot for a total of 10+ sessions. However, our experimental protocol departs from that traditionally used in HRI studies (excepting Björling and Rose \cite{bjorlingExploringTeensRobot2020} whose methods we look to replicate) in that our participants knew the robot was ultimately being controlled by the RC who was in the room and accessible for interaction. Participants were coached to avoid such interactions (based on their understanding of what we were trying to achieve with our ML system), and the room setup was designed to discourage it, with the RC seated out of the line of sight of GMs per Figure~\ref{fig:training}. Therefore, before discussing the impact of the robot, we first comment on participants perceptions of/interactions with the robot as an independent social agent versus an interface or accessary to communication with the RC.

\subsection{Do teens interact with the robot, or the RC?}
Observations of the group training sessions (which were primarily unsupervised but also video recorded for post-hoc analysis) suggest groups generally followed this protocol and engaged with the robot, rather than the RC, most of the time. However, we did see some interesting emergent behaviour around this, e.g. in one instance where the group could not agree on something, they asked the question to the robot and turned to the RC to indicate he should take the deciding vote but specifically via the robot, who they interacted with in terms of asking for/receiving the RC's decision. In this case, the RC role essentially appeared to represent an alternate form of group membership. 

We probed this explicitly during Focus Group 2 (day 9) asking how participants perceived the robot and the RC, given the RC-robot control/teaching setup. Further comments about how it felt to be the RC reinforced this idea of group membership: \textit{``I like it because I can do things that I thought would be needed when I was in the group.''} (R1) \textit{``It's like you can be a part of the discussion without really being a part of the discussion. It's like a ghost almost."} (W3). As GMs, participants generally described thinking about the robot as if it was `it's own person' until it did something `wrong': \textit{``I can say something dumb and then the robot disagrees with me, I'm like oh it's just W4 messing with me"} (W6) \textit{``if the robot says something we don't agree with, we turn to the person''} (B1) \textit{``Yeah, only when [the robot] goes wrong"} (B2). This concept of the RC/robot doing something `wrong', including participants' reflections on this and its potential implications for our approach are discussed further under RQ3. 

% [this ties in with kids ideas on enjoying the controller role still feeling part of the group, both for fun but also really reflective/wanting to help the group when controlling the robot]

% \textit{``I like it because I can do things that I thought would be needed when I was in the group.''} (R1)

% \textit{``It's like you can be a part of the discussion without really being a part of the discussion. It's like a ghost almost."} (W3) 


% \subsubsection{First Impressions}
% [some comment on initial experiences/impact etc, i.e. before the 'after a few days' comments given below? can be taken from qualitative forms ]

% \subsubsection{Midway Through Testing}

% As the Robot Controller is present in the same physical space as the group, we asked teenagers but also observed whether the robot was perceived as the robot or rather an extended version of the Robot Controller. Observations of the group training sessions (which were primarily unsupervised but also video recorded for post-hoc analysis) suggest groups generally followed protocol with respect to engaging with the robot rather than the Robot Controller most of the time. We did see some interesting emergent behaviour around this, e.g. in one instance where the group could not agree on something, they asked the question of the robot and turned to the Robot Controller to indicate he should take the deciding vote but specifically via the robot, who they interacted with in terms of asking for/receiving the Controller's decision. This raises the interesting notion of the Robot Controller role as an alternative form of group membership, and to what extent this in itself might be used as a group improvement mechanism, which we hope to explore in future work. 

\subsection{Does the robot impact the group, and (how) does this change over time?}
Concerning the impact of the robot on group working, R2D2 generally described being impressed by what the robot could do, but also feeling that the robot was less helpful now compared to in the beginning because they know each other better and already work together quite well as a group. \textit{``Mine are much more positive for robots. I think that they can actually help to like recover a bad discussion and also I feel like it has more potential than I thought in the beginning''} (R2) \textit{``I feel like it's gotten less helpful. Just because we got to know each other"} (R4) \textit{``Yeah, maybe sometimes it still helps. When it's like asking someone for an opinion, I think but it's much more rare these days''} (R2).

This sentiment was also echoed to some extent in Baymax, but more with respect to group members becoming less hesitant to speak during group activities and hence less in need of prompting. However, they also identified ways in which they felt the robot did still actively help, specifically the management of turn taking and keeping the group focused. \textit{``I think that it still is helpful because it can still help with who's going to talk now. Maybe this person has been a little bit talking. This person has been quiet. It gets focused, get back to like the topic. I think it's still like really good like that, but I think that it that's not that much necessary anymore, because now everybody is talking"} (B2) \textit{``Yeah, I also think that the robot it’s pretty helpful. Because if the group is not focusing then it can actually help the group to focus''} (B3) \textit{``It's helpful, but not as much anymore''} (B5).

% \subsection{Day 8: Reflections on the Summer School}

% \subsection{Day 9: Robot Removal}

% \subsubsection{On Robot Removal}
\input{tables/removal_comments}

The impact of the robot is also evidenced by students' comments and session evaluations after undertaking group activities \textit{without} the robot on Day 9; exemplars of which are provided in Table~\ref{tab:norobotsessions}. %provides a selection of scores and comments from session evaluations completed after undertaking group activities without the robot on Day 9. 
Comments made in brief group interviews after undertaking these sessions without the robot seemingly reflect and reiterate those evaluation scores and comments presented in the table. R2D2 maintained their initial feeling that they did not really \textit{need} the robot, but noted it improved their enjoyment: \textit{``These last days it has like worked well even like the robot hasn't had the need to do much. So it wasn't like it a worse discussion, but it's more fun when the robots there. So you get like more energy."} (R2) \textit{``Exactly"} (R1).

Wall-E had mixed opinions, seemingly the impact of the robot varied depending on which three participants took the GM roles. For example (W4, observed to be very much engaged with wanting to complete the group task) lamented the robot's absence after conducting group work with two of her less task-engaged group mates: \textit{But you know who you are, they kept on arguing, right? Yeah, and the robot could have stopped that, yeah, so I had to... The robot could have said like focus up. Or something to make them stop, but there was no robot so I had to try to stop them and it didn't work so.''} (W4) \textit{``I mean, it depends on we are not always in the same group. Different groups work different"} (W1). One Wall-E member specifically raised an interesting idea here regarding the robot actually being \textit{more} important now for groups who know each other rather than for groups working together for the first time, which was at odds with their own previous ideas (as well as R2D2s comments) on where such a robot might be most helpful: \textit{``If you know people very well, I think it would help like more than if you do not know them very well... because in first time interactions you wouldn't be like screaming at them, you would be a little calm to get to know them.''} (W5)

Finally all Baymax members seemed to agree that the robot was very necessary in helping them to work together, noting that they really did not work well together at all in these sessions without it: \textit{``The robot, always reminds you focus, do things, ask questions, but now they just like, it's so easy to just don't work."} (B4) \textit{``I think that it was really like a lot of people just like lost focus and started talking about something else. I was the only one working, actually."} (B2)

% Together with the evaluations provided in Table~\ref{tab:norobotsessions} these comments provide further evidence for our conceptualisations of the groups as being along a spectrum with regards to their need/use of the robot, ranging from the robot not really being \textit{needed} but still somehow adding to the experience (R2D2) to the use/necessity of the robot really varying based on the specific sub-combination of group members (Wall-E) to the robot really playing a key role in helping the group work together (Baymax). 

% \subsection{Impact on Participants}

% One-sided paired t-test analysis demonstrated a statistically significant decrease in participants' negative attitudes towards robots (T = 3.15, p $<$ 0.01) but also their group skills (T = 2.46; p = 0.01). The result on group skills goes somewhat against our hypothesis that taking part in the summer school would \textit{increase} participants' group working skills; however we believe this result might actually reflect participants being more aware of/better able to reflect on their behaviour in groups, hence answering the survey more honestly, rather than an actual decrease in group working skills.  

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.9\linewidth]{nars.png}}
% \caption{Comparison of pre- and post-hoc scores on the Negative Attitudes towards Robots (NARS) scale~\cite{syrdal2009negative}. Students demonstrated a significant decrease in their negative attitudes towards robots after taking part in the summer school.}
% \label{fig:nars}
% \end{figure}

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.9\linewidth]{groupskills.png}}
% \caption{Comparison of pre- and post-hoc scores on our group skills measure. Results suggest a significant decrease in group skills, but we believe this more likely reflects an increase in understanding and/or self-reflection on their behaviour when working in a group}
% \label{fig:groupskills}
% \end{figure}


==> sections/results_rq3.tex <==

\section{Reflections on the Pros, Cons and Practicalities of Our Approach (RQ3)}
\label{sec:rq3}

Firstly, all participants appeared to value our pursuit of their involvement our design and development process, with some referring generally to the importance of end-user involvement and some more specifically referring to their personal involvement in the design of robot for \textit{them}, noting that it's fun to see actions designed by themselves or their group members `in action'. \textit{``I feel like if it's just adults...they didn't do the same things as teenagers as we do now, so. I feel like you need to get close with people who actually like or in that age group.''} (R3) \textit{``I think it's important that we designed it."} (B4) \textit{``It's funnier to say something that you had decided''} (B1). This in itself is a strong motivator for pursuit of such approaches (as it points towards potential positive impacts on acceptability and effectiveness) and points towards further study of \textit{peer} versus \textit{self} designed robots in this context. Here however we reflect more specifically on our application of LEADOR and lessons learned for teen-in-the-loop design/automation more generally.

% \textit{``I would prefer to do it myself. Or like if it if it's like this. If it's like this that it's also other kids, but like I'm also in the group''.} (B2) 
\subsection{Could LEADOR be a feasible way to approach the automation of social robot behaviour with teens?}

Between days 9 and 10, we trained a simple ML agent based on the training data collected. This allowed participants to experience and evaluate a first attempt at autonomous robot behaviour based on the data they had generated over the course of the summer school. Whilst detailed evaluation and critique of that initial ML model is out of scope for this paper, we observed that it worked relatively well except for disproportionately executing the \textit{Disagree} action. Further work is required to disentangle the extent to which this reflects e.g. our specific choice of algorithm versus (excessive) use of that action during training sessions. 
%The action distributions in Figure~\ref{fig:actionsgroups} combined with the qualitative data regarding which actions the RC used when and why make the latter difficult to assess, as the \textit{Disagree} action was not used infrequently, but 
%This most likely reflected our choice of ML algorithm more than the training data set; as shown in Figure~\ref{fig:actionsgroups} there is no evidence to suggest, overall, participants disproportionately used the \textit{Disagree} action when taking on the RC role.
However, on observing this, participants quickly surmised that certain RCs might have biased the ML agent by over-utilising the \textit{Disagree} action - not with the intention of biasing the agent, but as a way of teasing their group members, again linking to RC as form of group membership discussed under RQ2. 

\subsection{Who should be `allowed' to train the robot?}

Given participants' own summations on the use of the \textit{Disagree} action, we probed them then on \textit{who} exactly should be involved in training the robot to be autonomous i.e., whether we should collate \textit{everyone's} training data or only that of select RCs (or even ourselves) who were most likely to refrain from doing anything `silly' and model exemplar group assistant behaviour. 
%to reflect on the impact on how choices made by the RC could influence the resulting, autonomous behaviour: they quickly started speculating about whether certain RCs might have biased the ML agent by (intentionally, for fun) over-utilising the \textit{Disagree} action (a behaviour observed once or twice towards the end of the study whereby certain RCs seemed to use this as a way of teasing their group members - linking to RC as form of group membership discussed under RQ2). This allowed us to probe participants thoughts about who then should be involved in \textit{training} the robot to be autonomous i.e., whether we should collate \textit{everyone's} training data or only that of select RCs (or even ourselves) who would avoid such behaviour. 
Whilst the R2D2 group poked fun at one group member as being one of those RCs who was indeed perhaps over-enthusiastic in their use of the \textit{Disagree} action in the final few sessions, they were also hesitant to lose such behaviour completely: \textit{``I feel like it's important to have [training data] from everyone but maybe like taking away *some* of the things [everyone laughs] like 50\% of the disagreement''} (R1) \textit{``I feel like some disagreement is good."} (R3) \textit{``And I feel like even though we all teach it differently, I feel like everything works for everyone. Like you can understand why someone may do a certain action. It's different ways but still working the same way."} (R2) \textit{[would it have been better if we researchers controlled the robot then?] ``No. Because like you guys are a lot older than us. As a kid, it's easier to understand the interaction maybe.} (R5) \textit{``Yeah I feel like you would have made the robot to a teacher more than a group member.''} (R1). This was echoed by the WALL-E group, who specifically suggested these (arguably) somewhat mischievous actions by the RC might ultimately prove crucial for robot acceptability and impact: \textit{``If I had a serious robot in front of me like I'm working with my friends or a group and...he's talking like OK, do this do that. Yeah, I would be bored, but if it's like a fun robot that takes it serious in a way, but it's still like a fun guy, that would change the whole perspective."} (W4). Perhaps hinting towards the ideal co-design scenario, one student in Baymax did wonder if there might be some way to `get the best of both worlds' by combining the data and ideas they generated with some from ourselves: \textit{``Because you guys know a bit more like how to train it. But I think it's a bit more fun for us if we get to like also programming the robot...maybe it was a bit better if it was both of us somehow"} (B2);  another direction worthy of consideration in future work.

% \subsection{What was participants' experience of the training process?}

On the training process more broadly, almost all participants identified a preference for being the RC or a GM rather than the GO during a training session; mostly finding the GO role to be the most boring. Unsurprisingly, it did not seem to generate the same feeling of extended group membership compared to the RC, and knowledge that the data generated by the GO might also be used in the training of the robot (as they were repeatedly reminded) did not seem enough to motivate their engagement with it. GOs often did not seem to consistently track and document group behaviour, and were generally observed to be quite disengaged, seemingly just waiting to swap back in to the RC or GM role. As such, we would re-consider our implementation of the GO role, if including it at all, in future iterations of this process.

% The \textit{training} stage of the LEADOR method is fundamentally based on an assumption that the training examples generated by the RC will, the majority of the time, represent an optimal action policy we want the robot to replicate.  


% \subsection{Impact on Participants}

% One-sided paired t-test analysis demonstrated a statistically significant decrease in participants' negative attitudes towards robots (T = 3.15, p $<$ 0.01) but also their group skills (T = 2.46; p = 0.01). The result on group skills goes somewhat against our hypothesis that taking part in the summer school would \textit{increase} participants' group working skills; however we believe this result might actually reflect participants being more aware of/better able to reflect on their behaviour in groups, hence answering the survey more honestly, rather than an actual decrease in group working skills.

% It also seems to have been these mischievous actions that triggered the group members, when working with the robot, to remember or re-conceptualise the robot as actually being a vehicle for the robot controller, whereas generally they referred to thinking about the robot as if it was `it's own person':

% % \textit{``I can say something dumb and then the robot disagrees with me, I'm like oh it's just W4 messing with me} (W6)

% \textit{``if the robot says something we don't agree with, we turn to the person.''} (B1) \textit{``Yeah, only when it goes wrong.} (B2)

% [this ties in with kids ideas on enjoying the controller role still feeling part of the group, both for fun but also really reflective/wanting to help the group when controlling the robot]

% \textit{``I like it because I can do things that I thought would be needed when I was in the group.''} (R1)

% \textit{``It's like you can be a part of the discussion without really being a part of the discussion. It's like a ghost almost."} (W3) 

% >> can we say anything from our observations or from the videos about how often they did 'break the 4th wall' with the robot controller as per W6's comment: \textit{She had an idea for name, he had an idea for a name and he had an idea for a name, and I was controlling the robot and they told me their names and I made the robot say I agree with you W4.} (W6) and/or how much they appeared to conceptualise the robot as `its own person' <<

% More broadly on the co-design process, and building on the idea of teens as being better robot teachers than us researchers, all participants appeared to value our participatory co-design approach, in some cases referring generally to the importance of (generally) having the ultimate end-user involved, but also in some cases more specifically referring to them wanting to be personally and specifically involved, or it being fun to see actions designed by themselves or their group members `in action'. 

% \textit{``I feel like if it's just adults...they didn't do the same things as teenagers as we do now, so. I feel like you need to get close with people who actually like or in that age group.''} (R3)

% \textit{``I think it's important that we designed it."} (B4) 

% \textit{``I would prefer to do it myself. Or like if it if it's like this. If it's like this that it's also other kids, but like I'm also in the group''.} (B2) 

% \textit{``It's funnier to say something that you had decided''} (B1) 

% Perhaps hinting towards the ideal co-design scenario, one student in Baymax did wonder if there might be some way to `get the best of both worlds' by combining the data and ideas they generated with some from ourselves:

% \textit{``Because you guys know a bit more like how to train it. But I think it's a bit more fun for us if we get to like also programming the robot. But I think that maybe sometimes, yeah, it could be like also good if you guys do something for us. If we all can do plus. So that's my opinion that maybe it was a bit better if it was both of us somehow, maybe."} (B2)
